Ordering information on distributions

This thesis details a class of partial orders on the space of probability distributions and the space of density operators which capture the idea of information content. Some links to domain theory and computational linguistics are also discussed. Chapter 1 details some useful theorems from order theory. In Chapter 2 we define a notion of an information ordering on the space of probability distributions and see that this gives rise to a large class of orderings. In Chapter 3 we extend the idea of an information ordering to the space of density operators and in particular look at the maximum eigenvalue order. We will discuss whether this order might be unique given certain restrictions. In Chapter 4 we discuss a possible application in distributional language models, namely in the study of entailment and disambiguation.

==> FrontBackMatter/Acknowledgments.tex <==
%*******************************************************
% Acknowledgments
%*******************************************************
\pdfbookmark[1]{Acknowledgments}{acknowledgments}

\begin{center}{\slshape    
   It is difficult to avoid the impression\\ that a miracle confronts us here, \\
  quite comparable in its striking nature\\ to the miracle that  the human mind\\
  can string a thousand arguments together\\ without getting itself into contradictions,\\
  or to the two miracles of the existence of laws of nature\\ and of the human mind's capacity to divine them.} 
\end{center}
\medskip
\begin{flushright}
    %--- \defcitealias{knuth:1974}{Donald E. Knuth}\citetalias{knuth:1974} \citep{knuth:1974}
       --- Eugene Wigner, The Unreasonable Effectiveness of Mathematics in the Natural Sciences
\end{flushright}



\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax
\chapter*{Acknowledgments}
Bla bla, thank you and such.
\endgroup





==> FrontBackMatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Put your declaration here.
\bigskip
 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> FrontBackMatter/Dedication.tex <==
%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Dedication}{Dedication}

\vspace*{3cm}

\begin{center}
    \emph{Ohana} means family. \\
    Family means nobody gets left behind, or forgotten. \\ \medskip
    --- Lilo \& Stitch    
\end{center}

\medskip

\begin{center}
    Dedicated to the loving memory of Rudolf Miede. \\ \smallskip
    1939\,--\,2005
\end{center}

==> FrontBackMatter/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        


==> FrontBackMatter/Publication.tex <==
%*******************************************************
% Publications
%*******************************************************
\pdfbookmark[1]{Publications}{publications}
\chapter*{Publications}
Some ideas and figures have appeared previously in the following publications:

\bigskip

\noindent Put your publications from the thesis here. The packages \texttt{multibib} or \texttt{bibtopic} etc. can be used to handle multiple different bibliographies in your document.
